Segment-Based Test Case Prioritization: A Multi-objective Approach

Regression testing of software is a crucial but time-consuming task, especially in the context of user interface (UI) testing where multiple microservices must be validated simultaneously. Test case prioritization (TCP) is a cost-efficient solution to address this by scheduling test cases in an execution order that maximizes an objective function, generally aimed at increasing the fault detection rate. While several techniques have been proposed for TCP, most rely on source code information which is usually not available for UI testing. In this paper, we introduce a multi-objective optimization approach to prioritize UI test cases, using evolutionary search algorithms and four coverage criteria focusing on web page elements as objectives for the optimization problem. Our method, which does not require source code information, is evaluated using two evolutionary algorithms (AGE-MOEA and NSGA-II) and compared with other TCP methods on a self-collected dataset of 11 test suites. The results show that our approach significantly outperforms other methods in terms of Average Percentage of Faults Detected (APFD) and APFD with Cost (APFDc), achieving the highest scores of 87.8\% and 79.2\%, respectively. We also introduce a new dataset and demonstrate the significant improvement of our approach over existing ones via empirical experiments. The paper's contributions include the application of web page segmentation in TCP, the construction of a new dataset for UI TCP, and empirical comparisons that demonstrate the improvement of our approach.

==> cover-letter.tex <==
Dear ISSTA 2024 Program Chair and Reviewers,

We are writing to you to make a submission with the revision to our paper, titled 

“Segment-based Test Case Prioritization: a Multi-objective Approach”

that was submitted in the first round of ISSTA 2024 and requested for a major revision. We are greatly appreciative of the constructive feedback and comments from the reviewers of our paper. The suggested changes are as follows.

"This paper presents a novel TCP technique for Web Applications that exploits a notion of semantic similarity between Web Pages to prioritize tests. The reviewers appreciated the idea and the empirical evaluation, but they also identified several concerns that must be addressed before the paper can be considered for publication. The final decision is a major review round conditional to the following changes:

1. Provide a formal/mathematical discussion of the fitness

2. Explain how using the APFD metrics for both the fitness and evaluation metric is objective - i.e. this is a potential flaw in the experiment that they should address

3. Provide costs for segmentation in the paper

4. Provide runtime for the different algorithms"

We have addressed the suggested modifications from the reviewers as follows (In this cover letter, we are summarizing all those changes. The changes are highlighted in blue in the attached PDF file):

1. We have revised completely Section 3.3 on the Formulation for our Multi-objective optimization.

2. We have revised completely Section 3.3.4 on Fitness function with formal description and discussion.

3. We have added several paragraphs in Section 3.3.4 to explain how our fitness functions are defined and how they are independent of the APFD evaluation metric.

4. We also changed RQ2 to measure fault coverage, i.e., the Minimal Tests for Faults Detection (MTFD), instead of element coverage.

5. We have added Section 5.5 on time efficiency analysis for all the algorithms.

6. We have added Section 5.5.2. on the cost of segmentation.


Thank you,
Authors


==> major-revisions.tex <==
Decision
--------
2. Major revision

Meta-review
-----------
This paper presents a novel TCP technique for Web Applications that exploits a notion of semantic similarity between Web Pages to prioritize tests. The reviewers appreciated the idea and the empirical evaluation, but they also identified several concerns that must be addressed before the paper can be considered for publication. The final decision is a major review round conditional to the following changes:

1. Provide a formal/mathematical discussion of the fitness

2. Explain how using the APFD metrics for both the fitness and evaluation metric is objective - i.e. this is a potential flaw in the experiment that they should address

3. Provide costs for segmentation in the paper

4. Provide runtime for the different algorithms


%---------------------------------------------------------------
Response:

***All_Reviewers***

***Code and Data*** In our original submission, we also uploaded the supplementary materials  in the file ***segment-based-tcp-submission.zip***. The new dataset for UI test case prioritization is in ***data/test_suite_annotated***.

***Reviewer_A***

***RA_Q1*** ***Challenges*** There are several scenarios in which the source code of a web application may not be available for testing including 1) inaccessible front-end and back-end source code of third-party libraries, frameworks, APIs, 2) proprietary and legacy code, 3) Web applications hosted in remote servers, 4) unavailable code for business or security reasons, etc. Unlike test cases in unit testing, which are often coupled with the unit’s source code, test cases in Web/GUI testing are decoupled from the front/back-end code. Therefore, several Web/GUI test prioritization approaches rely on visual elements rather than underlying code. However, those state-of-the-art approaches discard semantics of the elements in a web interface and aim only to cover as many elements as possible early in testing. Many elements may be semantically related and behave functionally in a similar manner. Therefore, those approaches could prioritize  test cases that reveal the same failures, resulting in redundant coverage.

***Novelties*** While not requiring access to source code, our test prioritization approach for web applications focuses on visual elements to partition a web page into segments/regions (that contain semantically/functionally related/equivalent parts of the web page), and then attempts to cover as many segments as possible early in testing. Another novelty is the leverage of multi-objective optimization algorithms to balance different objectives regarding the coverages of segments (structure/hierarchy of objects), sibling objects, object types, and objects.

***RA_Q2*** The main ***technical contributions*** are the technique and formulation of Web/GUI test prioritization as a multi-objective optimization, aiming to reduce redundancy by considering above visual elements.

***RA_Q3*** For comparison, we chose as ***baselines*** the state-of-the-art GUI test case prioritization approaches that accept Web pages under testing as input. We exclude the approaches that leverage historical testing data. We followed the baselines’ papers/websites to re-implement their approaches.

***RA_Q4*** The ***dataset*** from Yandrapally_and_Mesbah_[34] is a state-of-the-art benchmark for Web testing published in 2022 with a large number of test cases, and coverage and passing/failing information.

***RA_Q5*** The configuration options include 1) population size [100, 200], 2) the number of generations [50, 100, 200, 500], and 3) crossover probability [0.3, 0.5, 0.8]. After running 10 times with different settings, we selected the best setting that gives balance between the running time and the fitness values (Section_4.5.2).

***Reviewer_B***

***RB_Q1*** ***Cost/effort to perform segmentation*** Our approach uses the automated web page segmentation algorithm from [11]. For a web page, segmentation took about 2 seconds and is only required once for the first run. That algorithm with 71% F1-score leads to the saving of 10% and 30% testing effort to detect all the faults in comparison with the Greedy and Random approaches, respectively (see Minimal Test for Fault Detection in Table_3). Future experiments are required to study the impact of segmentation accuracy on our prioritization algorithm.

***RB_Q2*** Due to optimization, our algorithm took about 30-60 seconds for 100 test cases. Greedy algorithm took about 1 second.

***RB_Q3*** ***Fitness function and number of objectives*** Our goal is to optimize the coverages of segments, sibling objects, object types, and objects. We measure these objectives using the following corresponding metrics: Average Percentage of Segment Coverage, Average Percentage of Sibling Coverage, Average Percentage of Object-Type Coverage, and Average Percentage of Object Coverage. For each metric, we customize the APFD formula to be used as a fitness function for that objective as in Equation_5 (Section_4.3). The rationale is that the goal of APFD is to prioritize failed test cases, and similarly we aim to prioritize the GUI elements revealing the faults.

Our multi-objective optimization algorithm generates a list of pareto front (non-dominated) solutions. Each candidate solution has four values for four fitness functions. We employ multi-criteria sorting on the set of non-dominated solutions, with the sorting weights in the following objective order: segments, siblings, object types, and objects (Section_3.2.6).

***Reviewer_C***

***RC_Q1*** ***Projects for evaluation*** Two projects in Yandrapally_and_Mesbah_[34]’s dataset missed either the testing steps or the recorded HTML for each step, thus, preventing us from extracting coverage information needed for our algorithm. Therefore, we collected two additional projects for completeness and diversity. They are well-known projects for web testing evaluation containing tester-written test cases.

***RC_  Q2*** ***Code and Data*** See ***All_Reviewers***

***RC_Q3*** ***Fitness and objective functions*** See ***RB_Q3***

***RC_Q4*** ***Coverage information*** (Section_3.2). We extracted coverage information to compute the coverages for our four objectives: segments, siblings, object types, and objects.
